On the Conflict of Robustness and Learning in Collaborative Machine Learning

Collaborative Machine Learning (CML) allows participants to jointly train a machine learning model while keeping their training data private. In many scenarios where CML is seen as the solution to privacy issues, such as health-related applications, safety is also a primary concern. To ensure that CML processes produce models that output correct and reliable decisions \emph{even in the presence of potentially untrusted participants}, researchers propose to use \textit{robust aggregators} to filter out malicious contributions that negatively influence the training process. In this work, we formalize the two prevalent forms of robust aggregators in the literature. We then show that neither can provide the intended protection: either they use distance-based metrics that cannot reliably identify malicious inputs to training; or use metrics based on the behavior of the loss function which create a conflict with the ability of CML participants to learn, i.e., they cannot eliminate the risk of compromise without preventing learning.

==> brouillons/0bis-whiteboard.tex <==
\color{teal}{
\textbf{Skeleton written on board}

\begin{itemize}
    \item Intro
    \begin{itemize}
        \item Robustness is important
        \item Let's not repeat history
        \item CML and robustness: what's changing
        \item What we do and what are the contributions
    \end{itemize}
    \item Taxonomy of Robustness
    \begin{itemize}
        \item Existing robustness: what are the categories we define and what fits in them
        \item What is out of scope (will influence title): no threat model (naive, no adv, HbC, ...) + data driven + not applicable (certified, smoothing, ...) + crypto based (TO CHECK) + other def of robustness (reliability of communications) + A\&B
    \end{itemize}
    \item Bouh to distance
    \begin{itemize}
        \item Theory: $\tau<\Delta(m_0, m_\adv)/\delta(t)$
        \item Experiments
        \begin{itemize}
            \item Fixed $\delta$
            \item Dynamic $\delta$
        \end{itemize}
        \item Takeaway: the proxy they use for robustness is not sound, this is not the definition we are looking for
    \end{itemize}
    \item Framework + eval of B
    \begin{itemize}
        \item Games (rob + learning)
        \item Reduction
        \begin{itemize}
            \item Perfect Robustness (== no attack) implies no learning: S = D
            \item $\epsilon$-learning implies $f(\epsilon)$-robustness at max: we can quantify capability of decision ($\epsilon$-learning implies $D_i$ brings +$\epsilon$) good decision on D, bad on $D_i$ (if not, then do not learn) 
        \end{itemize}
        \item Experiments
        \begin{itemize}
            \item $D-D_i$ versus $\epsilon$ (homo versus learning)
            \item $\epsilon$ versus robustness
        \end{itemize}
        \item Takeway: behavior good for robustness, but the quality of evaluation is inversely proportional to learning possible  
    \end{itemize}
    \item Experiments need to span: 
    \begin{itemize}
        \item architecture
        \begin{itemize}
            \item model type
            \item size
        \end{itemize}
        \item use case
        \begin{itemize}
            \item (F)MNIST
            \item health
            \item cars
        \end{itemize}
        \item size of network: 9 on its own too small, >25?, lower for health/cars (check papers)
        \item \% of compromised users
        \item homogeneity of the network
        \item AGG rules / robust algorithms
    \end{itemize}
\end{itemize}
}

\color{black}

==> brouillons/3a-theory_bis.tex <==
Current choices of $\Delta$, $\theta^*$, and $\delta$, such as bounding the norm of updates~\cite{rofl}, cannot provide this this guarantee.

In distance-based robust aggregation, updates that are close to the reference point $\theta^*$, according to the metric $\Delta$, are qualified as benign, while updates that are further away, above a given threshold $\delta$, are considered malicious.

%More precisely, given such instantiation of $\mathcal{O}_\texttt{malicious}$, the advantage of the distinguisher $\userD$ in winning the R-IND game is:
%$Adv_\userD^\text{R-IND}(\delta; S_\userD, \mathcal{D}) = 0.5$: within a radius $\delta$ they cannot distinguish malicious updates better than random. 


%Assuming that, after one epoch, the state changed, we can assume that the zone covered by $\Delta(\theta, \theta^*)<\delta$ changed, i.e., the zone is not the same to enable progress. 
%So, it is not sufficient that the participants are able to win the R-IND game, but need to win a \textit{composition} of R-IND games, i.e., if the composition of ``benign'' adversarial contributions also ``benign''?

%However, we find that in order to get to choose $\Delta$, $\theta^*$, and $\delta$ that fulfil this guarantee, it requires the same knowledge as the one needed to win the L-EUF.
% While we show that current choices of $\Delta$ and $\theta^*$ for distance-based metrics do not guarantee that accepted updates come from honest users only, it would be interesting to explore (a) if it is possible to find better choices of $\Delta$ and $\theta^*$,
% %that accurately distinguish updates
% and (b) if finding those values requires the same information as the one necessary for learning, i.e., whether our Theorem~\ref{theorem:behavior} also applies to distance-based aggregators.
There are now two hypotheses to what's changing from one epoch to another: (a) either $R$ is designed such that the space of benign updates is consistent throughout the epochs, i.e., the set of updates is determined before training, or (b) the space of benign updates as defined by $R$ changes across the epochs. 
% To be noted that this is related but not equivalent to whether one or more of $\Delta$, $\theta^*$, or $\delta$ are updated at each epoch.
% Indeed, the updates of norm below 1.~\cite{rofl}, the space changes at each epoch given the current model.
% Indeed, the value , e.g., $\theta^*$ is the update produced by the user at the current epoch~\cite{scclipping}, or $\delta$ is a function of the consensus of users at the current epoch~\cite{krum}.
% In the later case, the composition is of further most importance because now, the composition of games must also be a safe space.

\begin{figure}
    \centering
    \begin{tikzpicture}

    \coordinate (cross1) at (0.,0.);
    \filldraw[fill=green, fill opacity=0.1] (cross1) circle (1cm);
    \filldraw[pattern=dots, pattern color=black] (cross1) circle (1cm);
    \draw[thick] (cross1) ++(-0.1,0) -- ++(0.2,0); 
    \draw[thick] (cross1) ++(0,-0.1) -- ++(0,0.2); 
    
    \coordinate (cross2) at (0.5,0.5);
    \draw[thick] (cross2) ++(-0.1,0) -- ++(0.2,0); 
    \draw[thick] (cross2) ++(0,-0.1) -- ++(0,0.2); 
    \filldraw[fill=green, fill opacity=0.1] (cross2) circle (1cm);
    \filldraw[pattern=north east lines, pattern color=black] (cross2) circle (1cm);

    \coordinate (cross3) at (1.4,.5);
    \draw[thick] (cross3) ++(-0.1,0) -- ++(0.2,0); 
    \draw[thick] (cross3) ++(0,-0.1) -- ++(0,0.2); 
    \filldraw[fill=green, fill opacity=0.1] (cross3) circle (1cm);
    \filldraw[pattern=grid, pattern color=black] (cross3) circle (1cm);

    \end{tikzpicture}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> brouillons/4a-learning.tex <==
%with games in the context of CML and reason about these two properties and how the games interact.

%We recall that the learning goal in (C)ML is to find a model that produces accurate predictions on the true distribution.
%This true distribution is typically not known by individual users, who have only access to a subset of the universe: their local dataset.
%Learning can be measured with the loss function $L$.
%Formally, the goal of learning is to find the model $m$ such that its expected accuracy on the true distribution $\mathcal{D}$ is minimized: $\underset{m}{\text{ argmin }} \underset{(x, y)\sim \mathcal{D}}{\mathbb{E}}[\mathcal{L}(m, (x, y))]$.


%In many applications, the local data held by users is not enough to find such model $m$ with good accuracy.
%Either because the local data is very limited in quality, quantity, or both, or because the users knows only certain labels (i.e., the user A only knows how to classify pictures of cats).
%A straightforward way to increase the performance of a model is to increase the amount of data the model is trained on. 
%CML allows to build a model that benefits from more training data, by letting users collaborate into building a model that has seen all local training data, and consequently increase its performance at the predefined learning task.

%Formally, the L-EUF game is as follows:

%We can compute a bound on the advantage $Adv^\text{L-EUF}_\adv(\epsilon; S_\adv, \mathcal{D})$ in wining this game using the training set $S_\adv$ and $\mathcal{D}$, and the value of $\epsilon$, for example with PAC learning, but this is beyond the scope of this work.
%To be noted that this game relates to a standard statistical setting of empirical risk minimization (ERM).

%\subsubsection{Learning capability}

% Indeed, the game can be played not only with the data of one user, but with \textit{all} the available data.
% This would imitate a centralized scenario. 
% The difference in advantage in wining the game with local data ($S_\adv$) compared to the game using all of the data captures how much the user can expect to learn from the others.


%In the case of behavior-based evaluation, the server is given some local data in order to evaluate updates.
%if server knows, wait for server to tell you (parallel with compute on your own from 4.2) if server does not know, then users are also }

%\note{Do we need to relax to $\cup_i \mathcal{D}_i$ instead of $\mathcal{D}$?
% We can relax the requirement to do good on the whole true distribution, by the requirement to do good on the distributions of users: $\cup_i \mathcal{D}_i$.
% This comes at the "best that can be done".}

\iffalse
\paragraph{Collaboration Advantage (L-COL)}
In order to measure the benefits of collaboration towards the learning task, we create another game, the L-COL.
During the L-COL game, the adversary is given not only their local data, but also the one of the other users, in order to model collaboration.
Of course in CML, data is never shared, thus this game acts as an upper-bound on the benefits of collaboration.
The game is formally defined in Game~\ref{fig:lcol}.

\begin{figure}[h!]
\centering
\begin{pcimage}
\procedureblock[linenumbering]{L-COL$_\adv(\epsilon; S_\adv, S, \mathcal{D})$}{%
\color{blue}
m \gets \adv (S_\adv \cup S) \\
\color{black}
\mathcal{L}^* = \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m, (x, y))]\\
\pcreturn \mathcal{L}_\adv < \mathcal{L}^* + \epsilon
}
\end{pcimage}
\caption{L-COL Game. The difference with the L-EUF game is highlighted in \color{blue} blue}
\label{fig:lcol}
\end{figure}

The game is similar to the L-EUF game with the exception of Line 1, highlighted in blue. 
In addition to the prior of the adversary $S_\adv$, they are also given 
Instead of one dataset, $n$ datasets are given to the adversary
This game is useful when used in comparison with L-EUF.
We evaluate how much better can the adversary succeed at the learning task when collaborating.
If the adversary can win L-COL but not L-EUF, or if $Adv_{L-COL}^\adv > Adv_{L-EUF}^\adv$, it means that collaboration is beneficial for the learning task. 
If the adversary can win both L-COL and L-EUF with the same probability, it means that the adversary can win without the other users, and does not benefit from collaboration.
\fi

==> brouillons/4b-robustness.tex <==
\subsubsection{Robustness (IN)Dinstinguishability (R-IND)}
 
During the robustness distinguishability game, the challenger gives a model $m$ and a dataset $S_\adv$ sampled from a distribution $\mathcal{D}$ to the adversary, and asks them to distinguish whether the model is robust or not.
The robust model is generated with the help of an oracle $\mathcal{O}_\texttt{robust}$.
This oracle, given a true distribution $\mathcal{D}$ and a value $\delta$, can generate a model $m$ such that $R(m) <\delta$.
The non-robust model is not generated by random sampling since it would trigger trivial wins.
Instead, we use a second oracle $\mathcal{O)}_\texttt{poisoned}$ which outputs, also given $\mathcal{D}$ and $\delta$, a model $m$ such that $R(m) > \delta$.
The adversary wins if they are able to distinguish between the two.
The game is formally described in Game~\ref{fig:rind}.

\begin{figure}[h!]
    \centering
\begin{pcimage}
\procedureblock[linenumbering, syntaxhighlight=auto]{R-IND$_\adv(\delta; S_\adv, \mathcal{D})$}{
b\sample\bin\\
m_0 \gets \mathcal{O}_\texttt{robust}(\mathcal{D}, \delta)\\
m_1 \gets \mathcal{O}_\texttt{poisoned}(\mathcal{D}, \delta)\\
b’ \gets \adv (m_b, S_\adv) \\
\pcreturn b=b’
}
\end{pcimage}
    \caption{R-IND Game}
    \label{fig:rind_}
\end{figure}

If the adversary wins the R-IND game, it means that they are able to distinguish robust from non-robust models on the distribution $\mathcal{D}$, using $S_\adv$ only.
This is equivalent to showing that there exists a correct evaluator of robustness on $\mathcal{D}$.
The concrete bound depends on the oracles, and how close to the $\delta$ value the models they produce are.

The mapping from the R-IND to the context of CML is quite similar to the learning game: the distribution $\mathcal{D}$ is the true distribution of the inputs, and $S_\adv$ the local training set of the adversary. 
We say that the user can distinguish robustness if \textbf{for all} implementations of $\mathcal{O}_\texttt{robust}$ and $\mathcal{O}_\texttt{poisoned}$, the advantage in winning the game is non-negligible.
The oracle $\mathcal{O}_\texttt{poisoned}$ can be instantiated with an attack technique, and $\mathcal{O}_\texttt{poisoned}$ with the updates produced by a genuine user.
Then the advantage is related to the attack success. 

However, in CML, there is no need to evaluate models, but updates.
The R-IND game can easily be adapted to evaluate updates.
These updates are to be applied to the current state of the model to improve it.
Hence the R-IND game can be played with the model resulting from the current state $m_{current}$ with the update to be distinguished applied to it.
For example, if the update produced by user $i$ $\theta_i$ is a gradient and the aggregation function is simply to add accepted updates, the game can be played with the model $m = m_{current} + \theta_i$.
The challenge is then to know whether $R(m) \leq \delta$ or $R(m) > \delta$. 




\iffalse
During the robustness distinguishability game, the challenger gives a model $m$ and a dataset $S_\adv$ sampled from a distribution $\mathcal{D}$ to the adversary, and asks them to distinguish whether the model is robust or random.
The robust model is generated with the help of an oracle $\mathcal{O}_\texttt{robust\_training}$.
This oracle, given a true distribution $\mathcal{D}$ and a value $\delta$, can generate a model $m$ such that $R(m) <\delta$.
Similarly to the L-IND game, the random model is simply a model sampled from the models' space. 
Again to avoid sampling a robust model by accident, we add a \textit{repeat-until} loop to assert that the random model is not also a robust model.
The adversary wins if they are able to distinguish between the two.
The game is formally described in Game~\ref{fig:rind}.

\begin{figure}[h!]
    \centering
\begin{pcimage}
\procedureblock[linenumbering, syntaxhighlight=auto]{R-IND$_\adv(\delta; S_\adv, \mathcal{D})$}{%
b\sample\bin\\
repeat \\
\t m_0 \sample \mathcal{M}\\
\pcuntil R(m_0) > \delta\\
m_1 \gets \mathcal{O}_\texttt{robust\_training}(\mathcal{D}, \delta)\\
b’ \gets \adv (m_b, S_\adv) \\
\pcreturn b=b’
}
\end{pcimage}
    \caption{R-IND Game}
    \label{fig:rind__}
\end{figure}


If the adversary wins the R-IND game, it means that they are able to distinguish a robust model on the distribution $\mathcal{D}$ from a random non-robust model using $S_\adv$ only.
This is equivalent to showing that there exists a correct evaluator of robustness on $\mathcal{D}$.

The mapping from the R-IND to the context of CML is quite similar to the learning games: the distribution $\mathcal{D}$ is the true distribution of the inputs, and $S_\adv$ the local training set of the adversary. 
However, in CML, there is no need to evaluate models, but updates.
The R-IND game can easily be adapted to evaluate updates.
These updates are to be applied to the current state of the model to improve it.
Hence the R-IND game can be played with the model resulting from the current state $m_{current}$ with the update to be distinguished applied to it.
For example, if the update produced by user $i$ $\theta_i$ is a gradient and the aggregation function is simply to add accepted updates, the game can be played with the model $m = m_{current} + \theta_i$.
The challenge is then to know whether $R(m) < \delta$ or if $\theta_i$ is a random update. 
\fi

==> brouillons/experiments.tex <==
iffalse
\begin{figure*}
    \centering
    \begin{tabular}{|r|r|r|r|r|r|r|}
     \hline
     \multirow{2}{*}{Knowledge} & \multicolumn{2}{c|}{Error Rate} & \multicolumn{2}{c|}{Hinge} & \multicolumn{2}{c|}{ERR }\\\cline{2-7}
      & Local Training & Learning Capacity & Acc. of decisions & FPR of decisions & Acc. of decisions & FPR of decisions\\\hline \hline
       \multicolumn{7}{|c|}{non-IID} \\ \hline
    0.1   & 90.2 & 87.4  & 0.042 & 0.75 &  0.035 & 1. \\
     0.2   &  78.9  &  76.1  & 0.08 & 0.5 &  0.059 & 0.55 \\
     0.5   & 49.0 & 46.2 & 0.094 & 0.947 &   0.091 & 0.2 \\
     0.8   & 21.4 &  18.6 & 0.122 & 0.846 & 0.168 & 0.143 \\
     0.9  & 12.26 & 9.46 & 0.143 & 0.533 &  0.491 & 0.042 \\
     1.    &  2.8  & 0 & 0.849 & 0.089 &  0.85 & 0.22 \\\hline

     \multicolumn{7}{|c|}{IID} \\ \hline
    0.001   & 57.83 & 55.03  & 0.56 & 0.406 &  0.448 & 0.59 \\
     0.01   &  78.9  &  76.1  & 0.635 & 0.315 &  0.494 & 0.369 \\
     0.1   & 49.0 & 46.2 & 0.712 & 0.277 &  0.609 & 0.207 \\
     0.5   & 21.4 &  18.6 & 0.841 & 0.121 & 0.853 & 0.064 \\
     1.    &  2.8  & 0 & 0.849 & 0.089 &  0.888 & 0.104 \\\hline
    \end{tabular}
    \caption{FPR}
    \label{fig:fpr}
\end{figure*}


\begin{figure*}
    \centering
    \begin{tabular}{|r|r|r|r|r|r|r|r|r|}
     \hline
     \multirow{2}{*}{non-IID} & \multicolumn{2}{c|}{Error Rate} & \multicolumn{3}{c|}{Hinge} & \multicolumn{3}{c|}{ERR }\\\cline{2-7}
      & Local Training & Potential Gain from Collab. & Acc. of decisions & FPR of decisions & Gain from Collab. & Acc. of decisions & FPR of decisions & Gain from collab\\\hline \hline
     %0.1   & 90.2 & -87.4  & 0.042 & 0.75 & 0.035 & 1. \\
    0.1   & 90.2 & -87.4  & 0.056 & 0.724 & & 0.035 & 1. & \\
     0.2   &  78.9  &  {-76.1}  & 0.08 & 0.5 & &  0.059 & 0.55 & \\
     0.5   & 49.0 & {-46.2} & 0.094 & 0.920 &  & 0.091 & 0.2 &\\
     0.8   & 21.4 &  {-18.6} & 0.122 & 0.846 & & 0.168 & 0.143 &\\
     0.9  & 12.26 & {-9.46} & 0.143 & 0.533 & & 0.491 & 0.042 &\\
     1.    &  2.8  & {0} & 0.849 & 0.089 & & 0.685 & 0.22 & \\\hline
    \end{tabular}
    \caption{Results}
    \label{fig:behavior_results}
\end{figure*}

\fi


\section{Health}

DISCO and HAM

https://arxiv.org/pdf/2009.08294.pdf and 

(1) The main task of this experiment is to learn federated models that
can predict the onset of the diabetes mellitus condition.
Dataset: We use the Pima Indians Diabetes dataset from the National Institute of Diabetes and Digestive and Kidney Diseases [15].
Data entries consist of medical measurements that correspond to
768 female patients older than 21 years old. These measurements
include diastolic blood pressure, body mass index, and plasma glucose concentration. Data is split into 614 samples for training and
154 for testing. The training data are shared among 10 federated
clients, where three of them own 39 samples, three own 59 and four
own 80. Client 1 is used as faulty, and clients (2, 4) are malicious.
Implementation: All the clients share the same neural network
(NN) model, which consists of 3 fully-convolutional (FC) layers
of size [200, 200, 2] neurons and combined with ReLU activation
functions. Local training epochs are fixed to 5 iterations, and 50
federated rounds. We use a learning rate of 1e − 5 with an Adam
optimizer, batch size of 10, and cross entropy as a loss function. The
client-level of the DP module is set to release 10% of the clients’
trained parameters, after adding the Laplacian noise with ϵ1 = ϵ3 =
1e − 4. The values of the DP parameters are set similar to [8]. For
the k-anonymity experiments, we set k arbitrarily to 4 with respect
to the age and pregnancies attributes. The value of k is usually
selected according to the data protection regulations that address
the training data usage.
Results: Figure 1a demonstrates the performance of different
aggregation methods with no bad clients. The results from the DP
experiments show that AFA and COMED can be more sensitive
than FA and MKRUM to the DP noise added to the local model
parameters. While the results from the syntactic approach with
k = 4 show a similar performance for all the models with a slightly
lower error rate for AFA and a higher one for MKRUM. Figure 1b
demonstrates the performance of different aggregation methods
with one faulty and one malicious clients. The results from the DP
experiments show that model trained using FA diverges compared
to the rest of the robust aggregation methods, while MKRUM performs the best. The results from the syntactic approach are similar
to the experiment with no faulty clients, despite the unstable performance of FA during the first rounds. 


\section{Driving}

https://arxiv.org/pdf/2302.08646.pdf and RobotCar dataset with YOLO (see https://www.kaggle.com/code/sudhanshu2198/yolov8-car-object-detection/notebook)

==> brouillons/graveyard.tex <==
%In other words, the user is given $m$ and asked to produce $\theta$ such that:
%$$ \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m+\theta)(x), y)] < \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m(x), y)] - \epsilon$$

%Resistance to invariance across environments (i.e., accurately classify a cow even if the background is not green)~\cite{invariance}, smooth classification of adversarial examples (i.e., correctly classify perturbed samples)~\cite{advex}, or good generalization (i.e., the quality of the model performance is the same on both seen and unseen examples)~\cite{generalization} are few examples of robustness considered in (C)ML.

One function is often not enough, so we want to make sure that across all functions that compare behavior this distance is small.
$$R(m) = \underset{\Delta: \mathcal{M}\times \mathcal{X} \rightarrow [0, 1]}{sup} \underset{x\sim\mathcal{D}}{\mathbb{E}}\Delta(m; x) - \Delta(m^*; x)$$


\iffalse
Naive aggregation is not robust with regards to its input, i.e., it is permeable to irregularities (which can happen with training data of poor quality) and attacks.
There exist more sophisticated aggregation functions, referred to as \textit{robust aggregators}, whose goal is to ensure a correct and accurate CML output, even in the presence of Byzantine users.
Robust aggregators limit (or fully discard) model updates that are believed to be detrimental to the learning process.
These robust aggregators are used by users during the aggregation step. %~\cite{ubar}.
% fi

This can also be seen as a distance metric (distance between two behaviors, just like Wasserstein distance for ex).

\iffalse
\begin{pcimage}
\procedureblock[linenumbering]{L-EUF$_{\mathcal{L}, \mathcal{D}}^\adv(\secpar)$}{%
S \sample \mathcal{D}\\
S_\adv \sample \mathcal{D}\\
m \sample \text{train}(S)\\
\theta \sample \adv (\secparam , m, S_\adv) \\
\mathcal{L} = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m(x), y)]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m+\theta)(x), y)]\\
\pcreturn \mathcal{L} > \mathcal{L}_\adv
}
\end{pcimage}

\begin{pcimage}
\procedureblock[linenumbering]{L-EUF$_{\mathcal{L}, \mathcal{D}}^\adv(\secpar, \epsilon)$}{%
S \sample \mathcal{D}\\
S_\adv \sample \mathcal{D}\\
m \sample \text{train}(S)\\
\theta \sample \adv (\secparam , m, S_\adv) \\
\mathcal{L} = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m(x), y)]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m+\theta)(x), y)]\\
\pcreturn \mathcal{L} > \mathcal{L}_\adv + \epsilon
}
\end{pcimage}
\fi



Parameterized by a function $R: \mathcal{M} \rightarrow \mathbb{R}$ and a quantity $\delta$.

$$M^{R, \delta} = \{m \in M | R(m) < 1-\delta\}$$



\subsection{Connection to CML}

Of course, in the collaborative setting, we are interested in the output(s) of users following the protocol. 
Users want to know if they learn from data or an update, i.e., if $\underset{x\sim\mathcal{D}}{\mathbb{E}} \mathcal{L} (m(x))$ is lowered, i.e., $\underset{x\mathcal{D}}{\mathbb{E}} \mathcal{L} (m'(x)) < \underset{x\sim\mathcal{D}}{\mathbb{E}} \mathcal{L} (m(x))$, where $m'$ is the model $m$ augmented with the data/update proposed. 
If the error is lowered, then the data/update is beneficial to learning, if not, then it does not help towards the learning task.

Defining what learning means is ok conceptually: you want to make the most correct predictions, (equivalently, minimal error), but tougher to formalize.

In particular, is learning the property of a model (i.e., this model learned this much) or is it the property of a step?
We rule out the fact that it is a property of training, nor data. 



\subsection{Definition}

We let learning be the property of a model.
This way, we can even extend the definition to a step by considering the difference in outputs before and after said step.
So, we let models fulfilling the $\epsilon$-learning property to be the set of models such that they are expected to have a loss below $\epsilon$, i.e.:

$$M^\epsilon = \{m \in M | \underset{x\sim\mathcal{D}}{\mathbb{E}} \mathcal{L} (m(x)) < \epsilon\}$$


Following, we define two games associated with the learning property. 
They will be useful later.

\paragraph{Learning Forgery (L-EUF)}

Game: given a state, the learning game asks the user to produce an update that satisfies $\epsilon$-learning.

\paragraph{Learning Dinstinguishability Game (L-IND)}

Game: given a state, the learning game asks the user to verify whether a model satisfies $\epsilon$-learning. 

Collaborative Machine Learning aims to be deployed in scenario where wrong predictions can cause safety issues, such as autonomous driving or health related applications. 
It is thus a primary concern to produce good and reliable decisions.
In the collaborative setup, it means that both contributions coming from (1) data of bad quality and (2) adversarial updates are filtered out.
To perform the filtering step, robust aggregators are used. 
The overwhelming majority of robust aggregators is based on distance, i.e., the quality of an update is deemed bad if it is further from a reference point by a given radius. 
In this work, we show that there is a fundamental trade-off between what can be learned and how much the final model can be manipulated, i.e., utility and robustness.

\section{Introduction}
Collaboration is a thing.
Applications include hospitals.
Security is a concern.
Actually, “Adversarial machine learning-industry perspectives,” in IEEE Security and Privacy Workshops, 2020. have revealed that robustness is considered the most feared threat faced today by companies that work with machine learning.
Security of a model is express through robustness.
Overall, the goal is to maximize the learning while minimizing unsafe behavior, i.e., the production of incorrect predictions.
However, we find that allowing learning directly implies allowing the possibility for adversaries to manipulate hence break robustness.
Any space given to progress cannot be controlled to be for good when learning.
We show an example with a big class of robust algorithm: distance based aggregators.

\section{What is robustness?}

\subsection{Formalization of robustness}
Robustness is a function of the predictions, i.e., behavior (or outcome) of the model.

We can test similarity in outputs compared to an ideal robust behaviour, or we can compare the models themselves. 
Comparing behaviors is tough, and usually it is not possible to test for all samples of the distribution. 
Hence, we should test on the models. 

Hence, robustness is a property of the model which produces the outputs.
Given an expected robust behavior, we can find models which have the desired property --- i.e., smoothness of the decision regions, or stability of prediction against distributions shifts.\\

Let's consider the \textit{set} of perfectly robust models $\mathcal{M}$ under the defined behavior.
We denote $\mathcal{M}'$ the result of training using a training set with distribution $\mathcal{D}$.
$\mathcal{D}$ can be arbitrarily different from an ideal and clean distribution, i.e., contains a subset of labels, or is a skewed distribution.\\
$R(M') = sup (X' \in P(X)) l(M'(X'), Y))$\\
The goal of robustness is to guarantee that when using any distribution $\mathcal{D}$, $\mathcal{M}'$ is as ``close" as possible to a robust and ideal model $\mathcal{M}_i$.
Beyond identity comparison (i.e., $\mathcal{M}_i$ and $\mathcal{M}'$ are the same), the notion of closeness is non trivial.
We generically denote it $\chi(\mathcal{M}_i, \mathcal{M}')$.
The closeness can act as a proxy for robustness. 
The closer $\mathcal{M}_i$ and $\mathcal{M}'$, the more robust $\mathcal{M}'$ is.
When equal, the closeness to an ideal model is maximized ($\chi=0$) and thus $\mathcal{M}'$ achieves maximal robustness. 
When the closeness is non-zero, the closer the functionality, the more robust.
The further away the functionality, the less robust.
Hence, robustness is not a binary concept but rather $\epsilon$-robustness.\\


Finding $\mathcal{M}$ is task dependant.
There exists more than one concept related to robustness in the ML literature.
Each can be used (or combined) to build a ground truth to whether a model is robust or not.
To be noted that it is not possible to check for the behavior of the model on the whole universe of samples.
Hence, the robustness that is found in the literature is often simplified to objectives that can be easily evaluated.
Definitions of robustness include (but are not limited to): maximizing the average accuracy performance; invariance under perturbations; or even performance on specific test samples. \\

Robustness can be formalized as a series of games:

\paragraph{Accept game:}
Given a contribution (i.e., a gradient) and a robustness threshold $\epsilon$, the accept game asks the user to either accept or reject a contribution, based on whether the contribution is a ``good" one (i.e., above $\epsilon$-robustness) or a ``bad" one (i.e., below $\epsilon$-robustness), again under the assumption that there exists a ground truth.

So, formally, given the set of ``good" contributions $\theta$ and bad contributions $\theta'$, the user must accept when given $\theta$, and reject otherwise.

This is equivalent to proving that there exist a verifier or that you can verify robustness. Not that you can efficiently find it.

\paragraph{Finding game:}
Given a robustness threshold $\epsilon$, the finding game asks the user to produce a contribution of at least $\epsilon$-robustness.

If there exist a user that can win the finding game, we can say that robustness can be produced efficiently.

\paragraph{Indistinguishably game:}
Given two contributions (i.e., two gradients), the distinguishing game asks the user to distinguish which one is the better one, under the assumption that there exists a ground truth, i.e., the one with $\epsilon$ with the most robustness.
So, formally, given $\theta$ and $\theta'$, the user must pick $\theta$.\\

This is more crypto, not sure yet.

\subsection{SoK: robustness in the wild}

What are the relationships between all notions of robustness?
For example: robustness to adversarial examples implies robustness to data shifts. 
Robustness to invariance implies robustness to data shifts.

It can be proven by looking at which are the good models given a rule, which itself can be used to reduce the games.

\subsection{Robustness in the collaborative setting}
When moving the the collaborative setting, the challenges are a bit different. 
It's not only about ensuring that no matter the distribution the model is robust. 
Now, participants receive updates from potentially untrusted users.
These users might be byzantine.
Given the criticality of the applications it is used in (health care, autonomous driving) malfunctioning would have disastrous consequences.
At the same time, there might be big incentives to influence the final model (e.g. to increase visibility of some content for advertisement applications). 
Hence, protecting the final model from being arbitrarily manipulated by adversarial participants is important.
The important translates in a lot of activity in the domain.
We stress that protecting from adversarial behavior protects from poor data quality with potentially incorrect labels.

\section{Insecurity of using $L_k$-distance as closeness metric}

\subsection{Distance-based approaches}
In this section we discuss the main trend in robustness in CML: using distance as closeness metric, hence as a way to evaluate robustness offered by an update.
Distance based aggregators can be generalized as:
$$\mathbbm{1}[||\theta - \theta^R||_k \leq \lambda].$$

The list includes Self Centered Clipping, where reference is own model and radius is predefined; RFA where R is the mean and the distance is a threshold; trimmed median where the reference is the median and the radius is the penultimate distance...

We denote the step size as $\lambda$.

\subsection{State-Override attack}

\paragraph{Threat Model:}
We use the standard Byzantine threat model.
We consider that there is \textbf{one} Byzantine user in the network $\adv$.
By definition, the Byzantine user is active, meaning that they are able to inject {maliciously} crafted updates into the network.
Under this model, the adversary is assumed to be omniscient, meaning that they know all messages sent on the network, and communication links and their weights.
In addition, the adversary has knowledge of public training parameters such as the learning rate.

\paragraph{Attack:} 
Formally, during the state--override attack, the Byzantine user sends:~$ \bm{\theta}_{\adv i} = \frac{\theta_{target} - \sum_{j \in \honestUsers} \theta_jW_{ij}}{W_{ib}}$
to each of its neighboring user $i$.

\subsection{Results}
\paragraph{Graphs and dataset} 
We use the MNIST dataset, split among users in a non--IID way to capture a more realistic setting.\footnote{Data is partitioned by class among the pool of users.}
We train a model with a shallow CNN architecture: layers = Conv-Conv-Dropout-fc-Dropout-fc; and using default training parameters: batch size = 32, momentum $\alpha$ = 0.9, learning rate $\eta$ = 0.01 without decay.

We consider 25 users, 24 honest and one Byzantine.
We use two different topologies to connect them: the torus and the complete topologies.
We assign equal weights to edges, i.e.,~$\bm{W}_{ij} = \frac{1}{|\mathcal{N}_i|}.$

We implement the State-Override attack on a range of distance-based aggregators.

\paragraph{exp1}
distance to target versus epoch

\paragraph{exp2}
accuracy on test set / epochs to get to target state versus step size. There should be a no learn zone and a no robustness zone.\\

\subsection{Discussion}
When allowing $\lambda$-learning, the adversary needs $\epsilon \leq \frac{||\theta_{target}-\theta^0||_2^2}{\lambda}$ epochs to get from $\theta^0$ to $\theta_{target}$.
If $\lambda$ is non zero, then this value is smaller than infinity and the adversary can get the model to the target state.

Conclusion: there is always an attacks, we show how to exploit.

\section{Generalization of the learning-robustness trade-off}

\subsection{Learning under robustness constraint}

\paragraph{Learning Game.}
Game: given a state, the learning game asks the user to produce an update that improves utility with at least $\epsilon$-robustness. 
So, formally, given a state $\mathcal{M}$ and $\epsilon$, the user must produce $\theta$ which improves the utility of $\mathcal{M}$.

\subsection{Learning $\Rightarrow$ Attack}
\subsection{No attack $\Rightarrow$ No learning}

The direction No learning $\Rightarrow$ No attack is trivial: do not learn by not accepting any change. 
In this case, there is no space for attack.

Let's look at the other direction now.
If one can win the accept game, i.e., the system is robust, then they can win the learning game.
Hence, they are not learning from the updates they accept.

\subsection{Discussion}
There is no $\chi$ such that it works. 
The only possibility is to consider the trade-off and understand which values of $\epsilon$ present a security risk or not.

Risk == one can find an attack: it is exploitable?

\section{Related work}

\subsection{Robustness attacks}
How:
Poisoning attacks compromise the training data.
Byzantine send bad gradients.

Target:
DoS-like aim to degrade the whole performance.
Back-doors are target specific.

\subsection{Robustness defenses}
Defenses can be applied during the whole pipeline. 
They can be system-y or ML-oriented.

If you can defend from during training, you can defend from pre-training, plus, during training is the same as defending after training.

In CML, since the updates can be malicious, during training is needed.


\subsection{On the distribution}

Given the ideal distribution $\mathcal{D}$ over the universe. 
Given a training algorithm $A$.
For the sake of the work, we assume $A$ is good.
We will expand on that later.
The model resulting from training on this data is ideal. 
We denote it $\mathcal{M}$.

Having an ideal distribution is not realistic, and in practice, the training is done using a distribution $\mathcal{D}'$.
$\mathcal{D}'$ can be arbitrarily different from $\mathcal{D}$, i.e., a subset, or skewed distribution.
When training using $\mathcal{D}'$, we denote the resulting model $\mathcal{M}'$.

The goal of robustness is to guarantee that when using the approximate distribution $\mathcal{D}'$, $\mathcal{M}'$ is as ``close" as possible to the ideal model $\mathcal{M}$, if possible the same.
The notion of closeness is not trivial.

Robustness using this formalization is impossible to achieve, i.e., there exist no $A$ that let the result of the training be $\mathcal{M}$ given any $\mathcal{D}'$.
%Of course, it is not possible to arrive to the ideal model $\mathcal{M}$ using any distribution arbitrarily different from the ideal one $\mathcal{D}$.

To relax the robustness, we denote $\mathbbm{M}$ the set of \textit{robust} models, and not just the ideal one.
These models are the results of training on the set of ideal distributions $\mathbbm{D}$.
We want $\mathcal{M}'$ to be in $\mathbbm{M}$ (and not just to be $\mathcal{M}$.

Furthermore, the closeness of $\mathcal{D}'$ to ideal distribution $\mathcal{D_i}$ should be related to the closeness of $\mathcal{M}'$ and $\mathcal{M}_i$.
Ideally, $\mathcal{M}'$ is $\mathcal{M}_i$ for $i$ such that $\mathcal{D}_i$ is the closest ideal distribution to $\mathcal{D}'$.
%Assuming that there exists a ground truth to whether a model is robust or not, we denote $\mathbbm{M}$ the set of robust models that can result from training on $\mathcal{D}$. 

We can then define $\epsilon$-robustness.


This can be done for example trough parametrisation, i.e., a model is evaluated as $\epsilon$-robust, and we say that the model is robust when $\epsilon$ is above a threshold. 

The $\epsilon$ can represent the distance to a robust model.
However, the set of robust models is not available and we need other things. 

The target can be granular, i.e., from the average performance on a given dataset to performance on specific test samples.
The way to measure robustness can then vary from one paper to another.

Given ground truth samples and labels, we define $(D, \epsilon)$-robustness of the model as the classification accuracy (or equivalently error) on the samples from distribution $D$, with $\epsilon$ radius smoothness.

Since the adversary could target any sample set, performance should technically be guaranteed on the whole distribution $D$.
However, it is not possible to check for the success rate across the whole universe. 
We can then use proxies:

$D$ = test set

$D$ = test set + radius around them

$D$ = a predetermined set targeted by adversary


\subsection{Connection}

The accept and distinguish games are equivalent.
If one can distinguish, one can accept.
If one can accept, one can distinguish.

If one can accept, one can win the learning game.

\section{Under the robustness constraint}

What can we learn under $\epsilon$-robustness?
Strictly speaking, robustness reduces the sets of models.

Since we can always forge D` such that M(D)=M(D`), we can have both.

\subsection{Learning Allowance $\lambda$}

If users want to learn, they must allow steps to be done from the starting point (if not, they do not learn). 
$$\lambda \leq ||\theta^T_* - \theta^0||_2^2$$

\subsection{Robustness Budget $\delta$}

At the same time, a bound on how much the adversarial users can influence is given by $\tau$.

If users want to learn, they must allow steps to be done from the starting point (if not, they do not learn). 
$$||\theta^{t+1} - \theta^t||_2^2 \leq \tau$$

so over $T$ epochs:

$$||\theta^{T} - \theta^0||_2^2 \leq T\cdot\tau$$

\subsection{$\lambda$ and $\delta$}

It does not make sense to allow more manipulation than learning. 
Hence the amount of manipulation is bounded by the learning allowance.



This is a lower bound since we need to consider that the adversary's unfiltered updates will propagate through the network according to the spectral graph of the underlying topology.

\section{Experiments}

\subsection{Experiment (1): given $\theta_{target}$, how many epochs?}
State-Override and sandtrap.


\subsection{Experiment (2): limited epochs, can we find the worse state?}

The assumption behind distance is that all state in radius $\tau$ are likely to improve.
We show that the adversary, for each epoch, can find something in this radius with worse performance.

==> brouillons/learning.tex <==
%\subsection{No Attack implies no Learning}
% \note{Perfect Robustness (== no attack) implies
% no learning: S = D}
% \textit{No attack} is the same as showing that the user can win the $R-IND$ game with $\delta=0$.
% Indeed, if the user can distinguish a robust update from a non-robust update, only the former are accepted, and as consequence, the model is 0-robust.
% When $R(m)$ is measured through the behavior of $m$, 0-robustness is equivalent to saying that $m$ behaves \textit{exactly} like the reference model $m^*$ on the true distribution. 
% We say that $m$ is perfectly robust. 
% Compared to the reference model $m^*$, there cannot be unspecified or unwanted behavior on inputs from $\mathcal{D}$.

% We know state the following: when $R(m)$ is measured through the behavior of $m$, an adversary winning the R-IND($0, S_\adv, \mathcal{D})$ game, the adversary has a learning capability of zero.
%The intuition behind the proof is that when the adversary wins the R-IND($0, S_\adv, \mathcal{D})$ game, it means that the adversary is able to distinguish a model (or update) that has 0-robustness from any other model (or update).
%The only way this is possible is when $S_\adv$ is representative of the true distribution, hence that the user can win the learning game.
% To sketch a proof, we start by having a look at the $R-IND$ game. 
% The challenge in producing correct evaluations is that the adversary does not $\mathcal{D}$, and only has access to a local dataset $S_\adv$.
% This is the only information available to the adversary, who needs to evaluate the behavior of $m$.
% It means that $R(m)$ is approximated by $\underset{x\sim S_\adv}{\mathbb{E}}\pi(m; x) - \pi(m^*, x)$, we call it $R^{S_\adv}(m)$.
%Meaning that models (or updates) will be accepted or rejected based on their behavior on a function of $S_\adv$.
%NOPE:If the adversary is able to produce correct decisions, it means that the behavior of $m$ is the same as $m^*$.
%%As consequence, any update that is accepted has behavior that is ``expected'' on $S_\adv$, thus that can be produced with $S_\adv$.
% If the adversary can win the $R-IND(0; S_\adv, \mathcal{D})$ game, they can always distinguish a robust update from a non-robust one.
% Then, $R^{S_\adv}(m)$ is a perfect estimator of $R(m)$.
% The only way this is possible is when $S_\adv$ is perfectly representative of $\mathcal{D}$.
% If $S_\adv$ is representative, this knowledge can be used to win the L-EUF($0, S_\adv, \mathcal{D}$) game.
% The next step in the proof is that, if the adversary can win the L-EUF($0, S_\adv, \mathcal{D}$) game without external updates, then, for any $S$, L-EUF($0, S_\adv \cup S, \mathcal{D}$) is not easier.
% In other words, when the adversary knows everything there is to know, there is no additional learning enabled by collaboration.
% For all $S$, Adv L-EUF($0, S_\adv, \mathcal{D}$) - L-EUF($0, S_\adv \cup S, \mathcal{D}$), which is the learning capability, is zero, at best negligible.
% This concludes the sketch of our proof.


%(a) if the updates is rejected, it trivially does not improve the learning, hence does not help with learning; and (b) If accepted, it means that the predictive capabilities of $m$ on $S_\adv$ behave as expected compared to the reference model.
%However, all information is contained in $S_\adv$, the update can be reproduced.
%Conversely, if the user want to truly learn, from the update, then they cannot evaluate robustness anymore, opening the door to attacks.
%The challenge of functionality-based robustness is to perform said evaluation with limited knowledge. 
%Let's first expand on what we mean by \textit{Learning}. 
%We refer to learning as the fact that a user will learn new information from collaboration.


\subsection{The cost of allowing learning}

The cost of learning

Let’s say that, given a delta, the adversary wins the R-IND game.
We build a R-IND game where the oracles are such that R captures the difference of malicious vs beginning, i.e., R < delta => benign and vice versa. 
The adversary can always evaluate theta on S, with the proxy R(theta, S).
However, it might not make good decisions on D\S.

It succeeds when it is a good proxy of R(theta, D), i.e., that S generalizes to D.
And fails when S does not represent D at all.

The advtange of wining R-IND is promotional to the represenativeness of S of D, modelled through epsilon.
 If S is representative, the adversary can correctly compute R and infer b.

Given an adversary that wins the R-IND game, we can construct an adversary that wins the epsilon game.
Indeed, under the assumption that S is epsilon representative, the adversary can craft theta that wins G(S_A, D)

The higher the advantage of A_IND, the higher the advantage of A_EUF.


In the context of CML.  Imagine there is a user such that S_an inter S_i = nul.
If the adversary can make a good decision on it versus not


Conversely, let’s imagine that there is S_i such that A_EUF (S inter S_I) > A_EUF (S). Then there exist a partition where S does not 

When the user makes perfect decisions, then S perfectly generalizes to D according to pi, and L-EUF can be won.

\mr{$\pi(\theta, S)$ composed with $\pi(\theta, D\setminus S)$}

\note{$\epsilon$-learning implies f($\epsilon$)-robustness at max:
we can quantify capability of decision
($\epsilon$-learning implies Di brings +$\epsilon$) good
decision on D, bad on D (if not, then
do not learn)}

First, we start with the assumption that the adversary cannot win the $L-EUF$ on their own, otherwise we would fall back in the ``no learning" scenario.
Then, we assume that there exists a dataset $S$, such that ADV L-EUF($\epsilon; S_\adv, \mathcal{D})$ - ADV L-EUF($\epsilon; S_\adv\cup S, \mathbf{D}$) is non-negligible.
%This difference, let's call it $\lambda$ captures how much the adversary learns from $S$, which we recall we call the learning capability, which in our context can also be seen as the \textit{collaboration advantage}.
%A large $\lambda$ indicates that the adversary can learn a lot from the network, while a small $\lambda$ suggests that there is less novel information.
We can conclude that there is a data partition of $\mathcal{D}$ spanned by $S$ that $S_\adv$ does not generalize to.
This in turn implies that the adversary cannot win the $R-IND(0; S_\adv, \mathcal{D}$ game since robustness decisions made on $S_\adv$ will not generalize either.
This gap is proportional to the learning capability of the adversary.
As consequence, learning entails lower quality of robustness decisions on the region you learn from.

%Learning is when the user could \textbf{not} win the $L-EUF$ game, but after collaboration, they can.}

%While the two statements (1) \textit{Learning $\Rightarrow$ Attack} and (2) \textit{No attack $\Rightarrow$ No learning} are equivalent, the later is easier to prove and argue about.

%While \textit{no attack} refers to the case where $\delta$ = 0, we can extend our claim to \textit{Bounded attack surface $\Rightarrow$ Bounded learning surface}, to consider $\delta$ > 0.

%However, updates that minimize the loss on $S$ have the same amount of information as $S$ itself. 

\subsection{Learning Games}

We recall that the learning goal in (C)ML is to find a model that produces accurate predictions on the true distribution.
This true distribution is typically not known by individual users, who have only access to a sub-sample: their local data.
Learning can be measured with the loss function $L$.
Formally, the goal of learning is to find the model $m$ such that its expected accuracy on the true distribution $\mathcal{D}$ is minimized: $\underset{m}{\text{ argmin }} \underset{(x, y)\sim \mathcal{D}}{\mathbb{E}}[\mathcal{L}(m, (x, y))]$.

In many applications, the local data held by users is not enough to find such model $m$ with good accuracy.
Either because the local data is very limited in quality, quantity, or both, or because the users knows only certain labels (i.e., the user A only knows how to classify pictures of cats).
A straightforward way to increase the performance of a model is to increase the amount of data the model is trained on. 
CML allows to build a model that benefits from more training data, by letting users collaborate into building a model that has seen all local training data, and consequently increase its performance at the predefined learning task.\\

%In CML, the purpose of learning comes from the fact that using local data only would lead to a model of poor performance. 
%Collaboration is seen as a way to improve the accuracy at the learning task.
%Learning is strongly associated with the loss function $L$ and more precisely how to minimizes it on inputs sampled from the true distribution $\mathcal{D}$.
%This is done through training, using a training set $S\sim \mathcal{D}$ and learning algorithm \textit{train}.
%For example, ERM finds
%$$\underset{m}{\text{ argmin }} \underset{(x, y)\sim S}{\mathbb{E}}[\mathcal{L}(m, (x, y))].$$

%In the collaborative setting, participants are motivated to collaborate because their local training data is limited, either in quality, quantity, or both. 
%The expectation from collaboration is to gain in performance over the true distribution, unknown to individual participants. 

%As consequence, the learning goal is to find a model that performs well over the true distribution.

%\note{Expand much more context: formalize the context and other users contribution instead of true distribution.}

%\subsubsection{Games}

In the following, we define a series of games associated with the learning property in the context of CML.  

\paragraph{Learning Forgery (L-EUF).}

First, we model the learning property through a forgery game, where the goal of the adversary is to succeed at the learning task.

More precisely, in the forgery game, the adversary is given a set $S_\adv$ sampled from a distribution $\mathcal{D}$ that is not shared with them, and challenged to forge (i.e., produce) a model with a loss $\epsilon$-close to the one of the optimal learner, on said distribution $\mathcal{D}$.
The challenger then checks whether the loss of the model returned by the adversary differs by less than $\epsilon$ from the one of the optimal learner.
If it is the case, the adversary wins the game.
The L-EUF game is formally described in Game~\ref{fig:leuf}.

%Formally, the L-EUF game is as follows:
\begin{figure}[h!]
\centering
\begin{pcimage}
\procedureblock[linenumbering]{L-EUF$_{\mathcal{L}, \mathcal{D}}^\adv( \epsilon)$}{%
S_\adv \sample \mathcal{D}\\
m \gets \adv (S_\adv) \\
\mathcal{L}^* = \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m, (x, y))]\\
\pcreturn \mathcal{L}_\adv < \mathcal{L}^* + \epsilon
}
\end{pcimage}
\caption{L-EUF Game}
\label{fig:leuf}
\end{figure}

The advantage of the adversary in winning the L-EUF game is tied to how well they are able to learn given their local data, i.e., succeed at the learning task.
In CML, $\mathcal{D}$ is the true distribution. 
\note{Do we need to relax to $\cup_i \mathcal{D}_i$ instead of $\mathcal{D}$?
We can relax the requirement to do good on the whole true distribution, by the requirement to do good on the distributions of users: $\cup_i \mathcal{D}_i$.
This comes at the "best that can be done".}
$S_\adv$ represents the training data available to users.
If the adversary can win with negligible probability, it means that an user in CML can learn a $\epsilon$-approximately correct model on the true distribution $\mathcal{D}$ using $S_\adv$ only.
The smaller $\epsilon$, the closer the model's performance is required to be to the one of the optimal learner.
The advantage of the adversary in wining this game is linked to the class of hypotheses, the training set $S_\adv$ and the value of $\epsilon$.
To be noted that this game relate to a standard statistical setting of empirical risk minimization (ERM).
A bound on $Adv^\adv_{L-EUF}$ can be derived from PAC learning.\note{Do we want to go there?}

\paragraph{Collaboration Advantage (L-COL).}

In order to measure the benefits of collaboration towards the learning task, we create another game, the L-COL.
During the L-COL game, the adversary is given not only their local data, but also the one of the other users, in order to model collaboration.
Of course in CML, data is never shared, thus this game acts as an upper-bound on the benefits of collaboration.
The game, defined in Game~\ref{fig:lcol}, is similar to the L-EUF game with the exception of Line 1, highlighted in blue. 
Instead of one dataset, $n$ datasets are given to the adversary.

\begin{figure}[h!]
\centering
\begin{pcimage}
\procedureblock[linenumbering]{L-COL$_{\mathcal{L}, \mathcal{D}}^\adv(\epsilon)$}{%
\color{blue} S_\adv = \{S_1, ..., S_n\} \sample \mathcal{D}^n\\
\color{black}
m \gets \adv (S_\adv) \\
\mathcal{L}^* = \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m, (x, y))]\\
\pcreturn \mathcal{L}_\adv < \mathcal{L}^* + \epsilon
}
\end{pcimage}
\caption{L-COL Game. The difference with the L-EUF game is highlighted in \color{blue} blue}
\label{fig:lcol}
\end{figure}

%\note{What happens if you give other users' data? If adv can ignore it yet still win (i.e., produce a model that has low loss on the true/union of users' distribution(s), then adv does not benefit from collaboration.}

This game is useful when used in comparison with L-EUF.
We evaluate how much better can the adversary succeed at the learning task when collaborating.
If the adversary can win L-COL but not L-EUF, or if $Adv_{L-COL}^\adv > Adv_{L-EUF}^\adv$, it means that collaboration is beneficial for the learning task. 
If the adversary can win both L-COL and L-EUF with the same probability, it means that the adversary can win without the other users, and does not benefit from collaboration.

\iffalse
Formally, the L-COL game is as follows:
\begin{pcimage}
\procedureblock[linenumbering]{L-COL$_{\mathcal{L}, \mathcal{D}}^\adv( \epsilon)$}{%
\{S_\adv = \{S_1, ..., S_n\} \sample \mathcal{D}^n\\
m_{\text{alone}} \gets \adv (S_\adv) \\
m_{\text{together}} \gets \adv (\{S_\adv, S_1, ..., S_n\}) \\\mathcal{L}^* = \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m, (x, y))]\\
\pcreturn \mathcal{L}_\adv < \mathcal{L}^* + \epsilon
}
\end{pcimage}
\fi

\paragraph{Learning Dinstinguishability (L-IND).}

Finally, we introduce a last game, the (in)distinguishability game, formalized in Game~\ref{fig:lind}.
In this game, the adversary is given a local data set and a model, and asked to distinguish a model that succeeds at the learning task from a random model.
The model that succeeds at the learning task is generated with an oracle $\mathcal{O}_\texttt{train}$ which given a distribution and a value $\epsilon$, can return a model $m$ such that its loss is $\epsilon$ close to the loss of the optimal learner on $\mathcal{D}$, i.e.: $\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m, (x, y))] < \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))] + \epsilon$.
The random model is simply a model sampled from the models' space. 
The probability of sampling a good learner as the random model is slim but non zero, and would bias the winning probability by making it impossible for the adversary to win.
A \textit{repeat-until} loop is added on the challenger side to ensure that the random model is not a good learner itself.


\begin{figure}[h!]
    \centering
\begin{pcimage}
\procedureblock[linenumbering, syntaxhighlight=auto]{L-IND$_{\mathcal{L}, \mathcal{D}}^\adv(\epsilon)$}{%
b\sample\bin\\
S_\adv \sample \mathcal{D}\\
repeat \\
\t m_0 \sample \mathcal{M}\\
\pcuntil \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m_0, (x, y))] > \epsilon \\
m_1 \gets \mathcal{O}_\texttt{train}(D, \epsilon) \\
b’ \gets \adv (m_b, S_\adv) \\
\pcreturn b=b’ 
}
\end{pcimage}
    \caption{L-IND Game}
    \label{fig:lind}
\end{figure}

If the adversary can win this game, it means that they are able to verify whether a model $m$ succeeds at the learning task on $\mathcal{D}$ by approximately $\epsilon$, only given a local dataset $S_\adv$.

We now explain the relation between the L-IND game and the L-EUF game and show that \textbf{winning L-IND $\Rightarrow$ winning L-EUF}.
We assume that there exist an adversary that can win the L-IND game.
Such adversary, denoted $\adv_{IND}$, is able to distinguish whether a model has learn up to $\epsilon$ on the true distribution, compared to the optimal learner, or is random,  given their local set.
An adversary $\adv_{EUF}$ who wants to win the L-EUF game can sample a model, use $\adv_{IND}$ as a black box to test whether this model is an $\epsilon$-good learner, and repeat until they find one.
When one is found, it can be used as an output to the L-EUF game.
The reduction is not computationally efficient, however, we note that the existence of a reduction has the implication that $S_\adv$ is \textit{enough} to win L-EUF, but that it is only a matter of computational power.
So, an adversary wining the L-IND game can also win the L-EUF game played on the same distribution with the same $\epsilon$ value with non-negligible probability. 

\note{Another direction: If $\adv$ can win L-IND with $S_\adv$, then $S_\adv$ is rep of $\mathcal{D}$: whenever the adversary is able to determine, given $S_\adv$ only, that an model has $\epsilon$-close loss on $\mathcal{D}$, $S_\adv$ is said to be representative of $\mathcal{D}$.
Then, given the PAC learning bound on representative dataset, we know that $S_\adv$ can be used to learn an approximately good model on $\mathcal{D}$, hence win L-EUF.}

\iffalse
Formally, the L-COL game is as follows:
\begin{pcimage}
\procedureblock[linenumbering]{L-COL$_{\mathcal{L}, \mathcal{D}}^\adv( \epsilon)$}{%
\{S_\adv = \{S_1, ..., S_n\} \sample \mathcal{D}^n\\
m_{\text{alone}} \gets \adv (S_\adv) \\
m_{\text{together}} \gets \adv (\{S_\adv, S_1, ..., S_n\}) \\\mathcal{L}^* = \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))]\\
\mathcal{L}_\adv = \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m, (x, y))]\\
\pcreturn \mathcal{L}_\adv < \mathcal{L}^* + \epsilon
}
\end{pcimage}
\fi


\paragraph{Learning Dinstinguishability (L-IND).}

Finally, we introduce a last game, the (in)distinguishability game, formalized in Game~\ref{fig:lind}.
In this game, the adversary is given a local data set and a model, and asked to distinguish a model that succeeds at the learning task from a random model.
The model that succeeds at the learning task is generated with an oracle $\mathcal{O}_\texttt{train}$ which given a distribution and a value $\epsilon$, can return a model $m$ such that its loss is $\epsilon$ close to the loss of the optimal learner on $\mathcal{D}$, i.e.: $\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m, (x, y))] < \underset{m^*}{\text{ min }}\underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}(m^*, (x, y))] + \epsilon$.
The random model is simply a model sampled from the models' space. 
The probability of sampling a good learner as the random model is slim but non zero, and would bias the winning probability by making it impossible for the adversary to win.
A \textit{repeat-until} loop is added on the challenger side to ensure that the random model is not a good learner itself.


\begin{figure}[h!]
    \centering
\begin{pcimage}
\procedureblock[linenumbering, syntaxhighlight=auto]{L-IND$_\adv(\epsilon; S_\adv, \mathcal{D})$}{%
b\sample\bin\\
repeat \\
\t m_0 \sample \mathcal{M}\\
\pcuntil \underset{(x, y)\sim\mathcal{D}}{\mathbb{E}}[\mathcal{L}((m_0, (x, y))] > \epsilon \\
m_1 \gets \mathcal{O}_\texttt{train}(D, \epsilon) \\
b’ \gets \adv (m_b, S_\adv) \\
\pcreturn b=b’ 
}
\end{pcimage}
    \caption{L-IND Game}
    \label{fig:lind}
\end{figure}

If the adversary can win this game, it means that they are able to verify whether a model $m$ succeeds at the learning task on $\mathcal{D}$ by approximately $\epsilon$, only given a local dataset $S_\adv$.

We now explain the relation between the L-IND game and the L-EUF game and show that \textbf{winning L-IND $\Rightarrow$ winning L-EUF}.
We assume that there exist an adversary that can win the L-IND game.
Such adversary, denoted $\adv_{IND}$, is able to distinguish whether a model has learn up to $\epsilon$ on the true distribution, compared to the optimal learner, or is random,  given their local set.
An adversary $\adv_{EUF}$ who wants to win the L-EUF game can sample a model, use $\adv_{IND}$ as a black box to test whether this model is an $\epsilon$-good learner, and repeat until they find one.
When one is found, it can be used as an output to the L-EUF game.
The reduction is not computationally efficient, however, we note that the existence of a reduction has the implication that $S_\adv$ is \textit{enough} to win L-EUF, but that it is only a matter of computational power.
So, an adversary wining the L-IND game can also win the L-EUF game played on the same distribution with the same $\epsilon$ value with non-negligible probability. 

\note{Another direction: If $\adv$ can win L-IND with $S_\adv$, then $S_\adv$ is rep of $\mathcal{D}$: whenever the adversary is able to determine, given $S_\adv$ only, that an model has $\epsilon$-close loss on $\mathcal{D}$, $S_\adv$ is said to be representative of $\mathcal{D}$.
Then, given the PAC learning bound on representative dataset, we know that $S_\adv$ can be used to learn an approximately good model on $\mathcal{D}$, hence win L-EUF.}

==> brouillons/numbers.tex <==
ER alone training (LR = 0.01) 7 cli (discard)
[90.2   6.49  4.89  5.02  7.42  6.18  7.56]
[78.86  6.15  5.13  4.93  7.14  5.94  7.36]
[49.04  6.12  5.28  5.08  7.58  5.87  7.5 ]
[21.39  6.12  4.98  4.94  7.55  6.08  7.64]
[12.26  6.61  5.46  5.29  7.58  6.37  8.95]
[2.82   6.39 5.24 5.19 7.03 6.11 7.52]

ER Hinge training (LR = 0.01)
[90.2   8.78  8.74  9.33  8.75  8.46  8.59]
[78.86 15.89 15.73 15.87 15.73 15.93 15.92]
[49.07 15.33 14.92 14.57 14.27 14.58 14.5 ]
[21.58 11.12 11.63 11.29 11.13 11.04 10.94]
[12.43  9.28  9.27  9.26  9.59  9.12  9.62]
[5.34 5.12 5.1  5.19 4.96 5.15 4.99]

==> brouillons/robustness.tex <==
\subsection{Robustness}

As we motivated above, in addition to having a model that is a good learner, it is also desirable to have robust outputs. 
As a general rule, the goal of robustness is to prevent errors from happening, equivalently, to ensure correct behavior of the model on any input from the true distribution.
Then, robustness is a function of a model.
We henceforth use $R(m)$ to refer to the robustness of the model $m$.
We say that a model $m$ is $\delta$-robust if $R(m)<\delta$.
We make the distribution the robustness is tested on implicit and embedded with the model to avoid the heavy notation $R(m, \mathcal{D})$.

While robustness in the centralized setting is already challenging, there is an added layer of difficulty in CML.
Indeed, users (or the server) receive model updates from participants.
These participants are not necessarily trusted to produce robust updates, i.e., updates that might be detrimental towards the robustness of the current state of the model and more generally of the CML output.
Hence, there is a need to evaluate the contributions proposed by other participants, and that without direct access to their data, in order to discard harmful contributions.
%This evaluation of robustness of updates coming from other users is a problem that is not necessarily related to privacy (which is the main goal of collaborative learning), but privacy makes it harder.
%It is not possible to look at the data to assert robustness. 
%But even in scenarios where privacy is not a concern, it would be still be hard to get robustness.\\
%Then, users need to decide on a robustness evaluation function $R$, and accept (parts of) received updates such that the resulting model has robustness $R(m)$ above a threshold (that can be locally determined).

%\subsubsection{Game}

Similarly to learning, we define a game associated with the robustness property in CML. 

\paragraph{Robustness (IN)Dinstinguishability (R-IND).}

During the robustness distinguishability game, the challenger gives a model $m$ and a dataset $S_\adv$ sampled from a distribution $\mathcal{D}$ to the adversary, and asks them to distinguish whether the model is robust or random.
The robust model is generated with the help of an oracle $\mathcal{O}_\texttt{robust\_training}$.
This oracle, given a true distribution $\mathcal{D}$ and a value $\delta$, can generate a model $m$ such that $R(m) <\delta$.
Similarly to the L-IND game, the random model is simply a model sampled from the models' space. 
Again to avoid sampling a robust model by accident, we add a \textit{repeat-until} loop to assert that the random model is not also a robust model.
The adversary wins if they are able to distinguish between the two.
The game is formally described in Game~\ref{fig:rind}.

\begin{figure}[h!]
    \centering
\begin{pcimage}
\procedureblock[linenumbering, syntaxhighlight=auto]{R-IND$_{\mathcal{L}, \mathcal{D}}^\adv(\delta)$}{%
b\sample\bin\\
repeat \\
\t m_0 \sample \mathcal{M}\\
\pcuntil R(m_0) > \delta\\
m_1 \gets \mathcal{O}_\texttt{robust\_training}(\mathcal{D}, \delta)\\
S_\adv \sample \mathcal{D}\\
b’ \gets \adv (m_b, S_\adv) \\
\pcreturn b=b’
}
\end{pcimage}
    \caption{R-IND Game}
    \label{fig:rind____}
\end{figure}

If the adversary wins the R-IND game, it means that they are able to distinguish a robust model on the distribution $\mathcal{D}$ from a random non-robust model using $S_\adv$ only.
This is equivalent to showing that there exists a correct evaluator of robustness on $\mathcal{D}$.

The mapping from the R-IND to the context of CML is quite similar to the learning games: the distribution $\mathcal{D}$ is the true distribution of the inputs, and $S_\adv$ the local training set of the adversary. 
However, in CML, there is no need to evaluate models, but updates.
The R-IND game can easily be adapted to evaluate updates.
These updates are to be applied to the current state of the model to improve it.
Hence the R-IND game can be played with the model resulting from the current state $m_{current}$ with the update to be distinguished applied to it.
For example, if the update produced by user $i$ $\theta_i$ is a gradient and the aggregation function is simply to add accepted updates, the game can be played with the model $m = m_{current} + \theta_i$.
The challenge is then to know whether $R(m) < \delta$ or if $\theta_i$ is a random update. 

==> brouillons/toadd.tex <==
Current choices of $\Delta$, $\theta^*$, and $\delta$, such as bounding the norm of updates~\cite{rofl}, cannot provide this this guarantee.
Depending on the choice of $\Delta$, even when $\delta=0$ attacks may be possible.
